Set-valued classification -- overview via a unified framework

Multi-class classification problem is among the most popular and well-studied statistical frameworks. Modern multi-class datasets can be extremely ambiguous and single-output predictions fail to deliver satisfactory performance. By allowing predictors to predict a set of label candidates, set-valued classification offers a natural way to deal with this ambiguity. Several formulations of set-valued classification are available in the literature and each of them leads to different prediction strategies. The present survey aims to review popular formulations using a unified statistical framework. The proposed framework encompasses previously considered and leads to new formulations as well as it allows to understand underlying trade-offs of each formulation. We provide infinite sample optimal set-valued classification strategies and review a general plug-in principle to construct data-driven algorithms. The exposition is supported by examples and pointers to both theoretical and practical contributions. Finally, we provide experiments on real-world datasets comparing these approaches in practice and providing general practical guidelines.

==> tex/notations_table.tex <==
\begin{tabular}{@{}ll@{}}
    \toprule
    \textsc{Notation}  &  \textsc{Signification}  \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % $[K]$ & $\{1,2,\dots,K\}$ \\
    % \fadedmidrule
    % $2^{[K]}$ & Power set of $[K]$ \\
    % \fadedmidrule
    % $|A|$ & Cardinality of finite set $A$ \\
    % \fadedmidrule
    % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $\mathcal{X}$  &  Input space  \\
    \fadedmidrule
    $\mathcal{Y}$  &  Label space  \\
    \fadedmidrule
    $\mathbf{P}$  &  Generic probability  \\
    \fadedmidrule
    $\mathbf{E}$  &  Generic expectation  \\
    \fadedmidrule
    $\Prob$  &  Distribution of $(\bsX, Y)$  \\
    \fadedmidrule
    $\Prob_{\bsX}$  &  Marginal distribution of $\bsX$  \\
    \fadedmidrule
    $p_k(\bsX)$  &  Conditional probability of $Y$ given $\bsX$: $\Prob(Y=k \mid \bsX)$  \\
    \fadedmidrule
    $p_{(k)}(\bsX)$  &  $p_k(\bsX)$ reordered in decreasing order: $p_{(1)}(\bsX) \geq \ldots \geq p_{(K)}(\bsX)$  \\
    \fadedmidrule
    $\Gamma(\bsX)$  &  Set-valued classifier $\Gamma : \class{X} \to 2^{[K]}$  \\
    \fadedmidrule
    $\data_n$  &  $n$ \iid samples from $\Prob$  \\
    \fadedmidrule
    $\data_N'$  &  $N$ \iid samples from $\Prob_{\bsX}$  \\
    \fadedmidrule
    $\dots$  &  $\dots$  \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \bottomrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
